Shattering the Ephemeral Storage Cost Barrier for Data-Intensive Serverless Workflows

Serverless computing is a popular cloud deployment paradigm where developers implement applications as workflows of functions that invoke each other. Cloud providers automatically scale function instances on demand and forward workflow requests to appropriate instances. However, current serverless clouds lack efficient cross-function data transfer, limiting the execution of data-intensive applications. Functions often rely on third-party services like AWS S3, AWS ElastiCache, or multi-tier solutions for intermediate data transfers, which introduces inefficiencies. We demonstrate that such through-storage transfers make data-intensive deployments economically impractical, with storage costs comprising more than 24-99% of the total serverless bill. To address this, we introduce Zipline, a fast, API-preserving data communication method for serverless platforms. Zipline enables direct function-to-function transfers, where the sender function buffers payloads in memory and sends a reference to the receiver. The receiver retrieves the data directly from the sender's memory, guided by the load balancer and autoscaler. Zipline integrates seamlessly with existing autoscaling, maintains invocation semantics, and eliminates the costs and overheads of intermediate services. We prototype Zipline in vHive/Knative on AWS EC2 nodes, demonstrating significant improvements. Zipline reduces costs and enhances latency and bandwidth compared to AWS S3 (the lowest-cost solution) and ElastiCache (the highest-performance solution). On real-world applications, Zipline lowers costs by 2-5x and reduces execution times by 1.3-3.4x versus S3. Compared to ElastiCache, Zipline achieves 17-772x cost reductions while improving performance by 2-5%.

==> 10-ack.tex <==
\section{Acknowledgements}
\label{sec:ack}

The authors thank the anonymous reviewers as well as the members of the EASE Lab at the University of Edinburgh for their valuable feedback on this work. 
% We are grateful to Shyam Jesalpura for figures. 
This research was generously supported by the University of Edinburgh, Huawei and by EASE Lab’s industry partners and sponsors including ARM, Intel and Microsoft.

==> 7-discuss.tex <==
\section{Discussion}
\label{sec:discuss}

% \update{NEW SEC}

\textbf{Compliance with non-ephemeral data transfers.} \shortn{} accelerates ephemeral data transfers, i.e., when the time between producing and consuming objects is smaller than the lifetime of function instances, prevalent in serverless applications (Figure~\ref{fig:blob_cdf}) but are also fully compliant with other types of data transfers. Examples of the latter may include data produced rarely and used extensively afterward, such as weekly re-training of an ML model for an inference service. \shortn{} leaves the choice of the actual transfer implementation to the providers, which can decide it statically upon deployment or at run time. For example, providers may add an optional \texttt{is\_ephemeral} argument to offload this choice to developers.  Alternatively, providers can continuously monitor the \shortn{} failure-retry rate and resort to conventional through-storage transfers -- transparently to the application code. 

\textbf{Leveraging specialized hardware and software.} Providers are free to tailor \shortn{} implementation further based on the availability of specialized hardware, such as RDMA and SmartNICs, optimizing for performance or cost further. The \shortn{} performance we demonstrate in \S\ref{sec:eval} is a conservative lower bound of what could be achieved with specialized hardware~\cite{andromeda} or software~\cite{google:snap}.

\textbf{Changes to the existing serverless infrastructure.}
\shortn{} requires changes to the underlying serverless infrastructure to enable direct transfers and the object namespace management, which can create concerns for its adoption and use. First, we prototype \shortn{} in an open-source Knative platform showcasing its feasibility production systems. 
Second, the recent adoption of Knative~\cite{knative} by many cloud companies, such as Google, IBM, VMware, Nutanix, and RedHat, for their commercial FaaS products marks a trend for open-source FaaS in production~\cite{knative-offerings}.
Third, \shortn{} also appeals to those cloud tenants who prefer to manage their own cloud infrastructure.
The increasing maturity of open-source software~\cite{knative,openfaas,fission} for serverless computing enables cloud tenants to purchase virtual machines or managed Kubernetes services and deploy their tailor-made serverless infrastructure to reduce their cloud expenses.
Such tenants can directly adopt the \shortn{} open-source artifact to further improve their application performance and cloud bills.
% , without waiting for their cloud provider to do so. 

==> Makefile <==
PAPER=ms
BIBCLOUDDIR=./bibcloud
DOCKER_EMU=--platform linux/amd64


all: clean pull $(PAPER).pdf bib push

pull:
	git pull

push:
	git commit -a -m "manual commit"
	git push

pp: pull push

clean:
	rm -f $(PAPER).pdf prepress.pdf *.aux *.fdb_latexmk *.log *.bbl *.blg \
		*~ *.dvi *.vrb *.nav *.snm texput.* *.synctex.gz
	docker run ${DOCKER_EMU} --rm -it -v ${PWD}:/workdir arkark/latexmk latexmk -C $(PAPER).tex

bib: 
	python $(BIBCLOUDDIR)/bibcloud.py $(PAPER)
	docker run ${DOCKER_EMU} --rm -it -v ${PWD}:/workdir arkark/latexmk bibtex $(PAPER)

$(PAPER).pdf:
	docker run ${DOCKER_EMU} --rm -it -v ${PWD}:/workdir arkark/latexmk latexmk -pdf \
		-interaction=nonstopmode -silent \
		-latexoption=-file-line-error \
		-latexoption=-synctex=1 $(PAPER).tex \
		&& touch $(PAPER).dvi || ! rm -f $@


==> bibcloud/dcsl-latex.tex <==


 
% this file is compatible with 
%  - the sigplanconf.sty 
%  - the SIG-ALT-FULL.CLS - VERSION 1.6
%  - also the USENIX conferences (osdi, etc)
%  - also ASPLOS (jpaper)

% v0.1 - 2018-06-20


% Comment/comment the lines to dynamically configure the file

\newif\ifcomments
%\commentstrue



% PACKAGES THAT MUST ALWAYS BE DEFINED ONE WAY OR ANOTHER

\usepackage{xspace}                         % auto-space mgmt for commands
\usepackage{subfig}                         % subfloat
\usepackage[normalem]{ulem}                 % sout
\usepackage{upgreek}
\usepackage{comment}                        % \begin{comment}
\usepackage{rotating}
\usepackage{graphicx}
\usepackage{multirow}


%USENIX conferences are just {article} -- requires this additional:
%
\makeatletter
\@ifclassloaded{sigplanconf}{
%sigplanconf only additions
\usepackage{gensymb}  %socc - celsius
}{
%else
\usepackage{cite} % automatically sorts the citations.  there is an optional [nocompress].

\@ifclassloaded{jpaper}{
% ASPLOS papers
}{
% USENIX papers (in practice)
\usepackage{gensymb}  %socc - celsius
\usepackage[usenames, dvipsnames]{color}
\usepackage{url}
}
}
\makeatletter



%% poor man's layout
%% when \usepackage{layout} .... \layout is broken

\newcommand{\printlayout}{{\bf The textwidth \the\textwidth; the columnwidth is \the\columnwidth}}

% HYPHENATION HELP

\hyphenation{user-space}

% GENERIC THINGS

\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\ie}{\textit{i.e.,}\xspace}
\newcommand{\egparen}[1]{(\eg~#1)\xspace}
\newcommand{\ieparen}[1]{(\ie~#1)\xspace}
\newcommand{\egp}[1]{\egparen{#1}}
\newcommand{\iep}[1]{\ieparen{#1}}

\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\twiddle}{$\sim$}
\newcommand{\microsecond}{$\upmu{}$s\xspace}
\newcommand{\nanosecond}{$ns$\xspace}

\newcommand{\myitem}{\noindent$\bullet\hspace{10pt}$}
\newcommand{\myparagraph}[1]{\vspace{1em}\noindent {\bf #1:}}
 
%DCSL


\newcommand{\edb}[1]{\noindent{{\bf \fbox{EdB:} {\textcolor{red}{\it#1}}}}}
\newcommand{\george}[1]{\noindent{{\bf \fbox{GP:} {\textcolor{blue}{\it#1}}}}}
\newcommand{\marios}[1]{\noindent{{\bf \fbox{MK:} {\textcolor{green}{\it#1}}}}}
\newcommand{\jf}[1]{\noindent{{\bf \fbox{JF:} {\textcolor{Peach}{\it#1}}}}}
\newcommand{\ag}[1]{\noindent{{\bf \fbox{AG:} {\textcolor{Gray}{\it#1}}}}}
\newcommand{\sam}[1]{\noindent{{\bf \fbox{Sam:} {\textcolor{cyan}{\it#1}}}}}



%make sure to always define in the main latex file
%\newcommand{\system}{\textsc{FOOBAR}\xspace}


==> old2-back.tex <==


\section{Background}
\label{sec:back}

% \dmitrii{
% open questions for this section:
% \begin{itemize}
%     % \item where/how to bring up that most transferred data among serverless functions is ephemeral
%     \item Should we quantify inline and S3 transfers on AWS (or on AWS and Google)?
%     \item how do we bring up the ephemeral storage prior work? or should we show the gRPC curve as the "upper bound" performance and talk about ephemeral storage in the related work?
% \end{itemize}
% }

\subsection{Serverless Computing Basics}
\label{sec:serverless_101}

%Serverless is the next dominant cloud architecture. Developers compose applications as a collection of functions, connecting them to events, e.g., clicks. 
%These functions are invoked as a result to a set of events, e.g. database update or an incoming HTTP request.
%, which can be written in a high-level programming language such as Python.% and need to communicate with each other.
% A serverless function takes the form of an HTTP server that executes the equivalent function upon arrival of an HTTP request.

%%%Serverless has emerged as an important cloud computing paradigm in which cloud service developers organise their application logic as a series of {\em stateless} functions and offload the infrastructure management and resources (auto)scaling entirely to the cloud providers.
%%%To implement a serverless application, developers combine multiple functions in the form of HTTP servers with corresponding user-defined handlers.
%%%Within an application, functions are connected in a {\em workflow}, in which they invoke and communicate with each other.

A typical serverless application is composed of multiple stateless functions connected in a {\em workflow}. Functions, deployed as HTTP servers with user-defined handlers, may invoke each other. 
%The stateless nature of serverless means that any input to a function must be propagated as part of the invocation or retrieved from storage (further discussed in \S\ref{sec:back-prior}).

Two aspects are central to serverless deployments. The first is autoscaling, whereby function instances are launched on-demand, based on observed load. Autoscaling affords extreme scalability and cost-efficiency, as idle functions are rapidly shutdown by the cloud provider. The latter is facilitated by the stateless nature of serverless functions. 

The second important aspect of serverless is the unavoidable communication between function instances in a workflow. Communication is endemic due to the stateless nature of serverless, which cannot hold or share state across invocations. This often places inter-function communication on the critical path, performance-wise, necessitating a low-latency high-bandwidth communication substrate. 

The quest  for high-performance inter-function communication is complicated by the autoscaling aspect of serverless, since a producer instance in a workflow might not know the consumer until the latter is invoked  by the producer. It is only at the invocation point that the cloud infrastructure picks either an existing instance of the consumer function or spawns a new one based on observed load. Thus, any optimizations to the inter-function communication substrate must respect the cloud provider's autoscaling policies. 

The rest of this section details the workings of the autoscaling infrastructure and inter-function communication options in today's clouds.


%Thanks to the built-in autoscaling of serverless clouds, serverless applications can enjoy virtually infinite scalability, which, however, falls short for the applications that exhibit a lot of inter-function communication in modern clouds~\cite{klimovic:understanding,pu:shuffling,sreekanti:cloudburst,fouladi:encoding}. The cortex of this problem is in the {\em stateless} nature of serverless functions, which cannot hold or share state neither across invocations nor across functions, without using a third-party storage service.

%While autoscaling storage services are available in any of the modern clouds, e.g., \dmitrii{AWS S3~\cite{XXX} and Google Storage~\cite{XXX}}, it is ill-suited for serverless applications. Comprising sporadic and short-lived multiple functions, serverless applications mostly use storage for transferring intermediate, i.e., ephemeral, data across functions~\cite{klimovic:understanding}. In contrast, existing cloud storage solutions are tailored to deliver cheap highly-available storage for long-running services.

%We argue that enabling fast and cost-effective data communication must be {\em serverless-native}, i.e., co-designed with the autoscaling serverless infrastructure. Currently driving solely the compute resources scaling, the autoscaling infrastructure should deliver high-speed data communication via autoscaling of the communication resources, e.g., network bandwidth. 

\begin{comment}
\dmitrii{STOPPED HERE}
%%%%%%%%%%%%%%% OLD VERSION 

% Indeed, prior work demonstrates the lack of efficient support for high-speed data communication in serverless clouds. 


% Based on the isolation guarantees they want to provide, different cloud providers deploy function instances as independent virtual machines~\cite{agache:firecracker} or as containers that run inside a virtual machine and collocate multiple functions that belong to the same tenant. \dmitrii{probably not important details for this paper}

The key advantage of serverless computing both from a cloud tenant and a cloud provider perspectives is autoscaling. In serverless, the application developers pay only for the invocations of the functions they deploy, being billed for the execution time and the memory footprint that their functions use. In the presence of traffic changes, the providers are responsible for scaling the resources allocated to the functions, by spawning additional instances of these functions or tearing down the idle ones. At any moment in time, a function may have any number of active instances, from zero to virtually infinity. Hence, functions are designed to be stateless, allowing any instance to execute the corresponding function's logic.

Delivering seamless autoscaling to serverless workloads is a crucial albeit challenging goal for cloud providers. First, prior work demonstrated that serverless workloads exhibit unpredictable bursty traffic patterns~\cite{wang:faasnet,shahrad:serverless}, which requires the infrastructure to take autoscaling decisions at a high rate. Second, functions may feature an arbitrary number of instances at any moment, which can neither hold nor share inter-invocation state, making it difficult to achieve high performance data communication across different functions in a single workflow. Prior work~\cite{klimovic:understanding} shows that most communicated data is ephemeral, i.e., inputs and outputs that functions pass from one to another. However, an instance of one serverless function is unable to pass this data to an instance of another function directly, because the actual destination of the transmission depends on the decisions of the autoscaling infrastructure.

\end{comment}


\begin{comment}
%Providers deliver automatic scaling of each function and charge the developers based on the amount of resources their functions use (CPU time and memory footprint). The providers scale functions resources horizontally, by adding and tearing down instances of each function. 
Independent of the deployment method, though, the main benefit of serverless computing both from a cloud tenant and a cloud provider perspective is autoscaling.
Instead of paying for their active virtual machines independent of the incoming load, in serverless, cloud tenants pay only for the function invocations, thus being billed at a much finer granularity.
Apart from the economic benefit, though, a serverless application can automatically scale based on the incoming load.
The stateless design enables cloud providers to spawn more functions instances as the incoming load increases.
% From a cloud provider perspective the small memory and CPU footprint of serverless functions, compared to virtual machines, enables better workload consolidation and leads to more efficient use of resources.


From the above we understand that autoscaling is the cornerstone of serverless computing.
Thus, cloud providers need to make timely and careful autoscaling decisions both to improve their infrastructure utilization but also to deliver potential service level agreements.
However, like for other datacenter services, serverless function invocation traffic is bursty~\cite{shahrad:serverless,wang:faasnet}, making the implementation of such an autoscaling mechanism a challenging goal.
To deliver the scalability promise, the providers design their system around a comprehensive autoscaling infrastructure, which includes continuous load monitoring, resources scaling, and load balancing.
\dmitrii{need to think about connecting with the next subsec a bit better?}

\end{comment}



% Challenges for providers: functions are staleless, with an arbitrary user logic, invocation frequency, and bursty traffic. Providers need to autoscale each function's resources. They do it horizontally, by adding and removing instances.

% Takeaways: autoscaling and pay-as-you-go are the key advantages and must be the cortex of the design.

\subsection{Serverless Autoscaling Infrastructure}
\label{sec:autoscaling}


%As seamless provider-based scalability is the main advantage of serverless computing, serverless autoscaling infrastructure is the cortex of the serverless system architecture.
We describe the operation of a serverless autoscaling infrastructure~(Fig.~\ref{fig:autoscaling_infra}) using the Knative~\cite{knative} terminology, since it resembles production clouds, in particular Google Cloud Run~\cite{google:cloudrun} and AWS Lambda~\cite{agache:firecracker}.
% , which is representative of AWS Lambda~\cite{agache:firecracker} and vHive/Knative~\cite{ustiugov:benchmarking,knative}.

The autoscaling infrastructure of serverless is designed to achieve two objectives. The first is responding to changes in load by spawning new function instances when the load increases and shutting down idle instances once the load drops. The second objective is minimizing queuing latency by balancing the load across the active instances. 
%needs to satisfy two goals. First, new instances can be requested at any point in time in response to a change in the traffic while idle instances should be recycled to free up the cluster resources. Second, the load should be balanced across all active instances of a function at any point in time. 

\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figures/background/autoscaling_infra.pdf}
    \caption{Operation of serverless autoscaling infrastructure.
    % \ed{Need to re-draw in the style of Fig.~\ref{fig:xdt-design}}
    }
    \label{fig:autoscaling_infra}
\end{figure}

Instance scaling and load-balancing decisions inherently rely on utilization metrics from the active function instances, gathered and stored with the help of the following two components. 
%To monitor the load of the currently active instances, cloud infrastructure must timely collect utilization metrics from each of the active function instances and timely react with new instance placement decisions. To implement this, serverless infrastructure depends on two main components.
Each function invocation traverses a provider-managed {\em queue-proxy} component, which is in charge of forwarding incoming requests to the function instance with which the queue proxy is co-located.
% \boris{You need to spell out that the RP is co-located with the instance. Also, the dotted lines in the figure are quite faint in my print-out and hard to see -- please make them a tad thicker.}
% This component, called MicroManager in AWS Lambda~\cite{agache:firecracker} and Queue Proxy~\cite{knative} in Knative, 
Queue proxy also collects and reports utilization metrics of that instance to the {\em autoscaler} control plane component.
The {\em autoscaler}
%(called Placement Service in AWS) 
monitors the load in front of each active instance and implements the scaling policy.  
% For example, Knative uses the number of function invocations, waiting for execution in front of each instance, as a metric.
% AWS Lambda allows not more than one request to be assigned to an instance at all times~\cite{aws:concurrency}.

To balance the load among all active instances of a function, serverless clouds employ a {\em load balancer} whose job is to steer requests to one of the instances. Every function invocation must traverse the load balancer, referred to as the {\em activator} in Knative. 
%(Worker Manager in AWS Lambda) 
% \sout{it is a load-aware L7 load balancer.}
The activator periodically receives updates from the autoscaler regarding the active instances and their current load.
If there is an incoming request for a function and there are no active instances available or all of them are busy, the activator needs to request new instances of that function from the autoscaler.
The autoscaler makes a placement decision and spawns a new function instance while the activator buffers the pending function invocation request.
Once the new instance is up, the activator steers the buffered invocation to the instance via its corresponding queue proxy. 

% Figure~\ref{XXX} describes the interaction between these three components...

This triplet of components, namely the queue proxy, the autoscaler, and the load balancer, work together to enable autoscaling of serverless functions. The rest of the serverless system is designed around this triplet to deliver seamless scalability to serverless application developers and efficient resource usage to cloud providers.

\begin{comment}
We explain the autoscaling infrastructure components and operation by describing the lifecycle of a function invocation, using vHive/Knative architecture~\cite{ustiugov:benchmarking}. 


% Functions are abstract, having from 0 to \textit{inf} instances. Hence, the HTTP load balancer must be on the critical path of every single invocation.

TODO: Introduce the LB and the tandem of the reverse proxy and the autoscaler.

Takeaways: key components are LB, RP, and autoscaler. None can be bypassed w/o sacrificing serverless advantages.
\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Serverless Communication Methods}
\label{sec:back-prior}

Any meaningful serverless application must combine multiple stateless functions that communicate with each other.
The resulting inter-function communication can significantly affect the performance of the entire serverless application. We next discuss the various inter-function communication mechanisms, including solutions deployed in production in today's clouds and proposals from the academic community.

\begin{comment}
\dmitrii{Need to add a paragraph : ..need to support two API types, namely passing-by-value and passing-by-reference (narration similar to the HotOS paper~\cite{wang:reference}).. Then, inline and storage-based are their current implementation in existing systems.

\boris{somewhere, need to have a discussion of push vs pull. Perhaps in Related Work,if you plan on having that section.}

Bring up programming patterns \cite{mahgoub:sonic} broadcast, reduction, invoke.
}
\end{comment}


% \subsubsection{Production Methods}
\subsubsection{Commercial Solutions}

% \edb{I WOULD CALL THIS SUBSEC "Commercial solutions}

Serverless clouds, e.g., AWS Lambda or Google Cloud Functions, provide two methods of data transfers: either inline as part of the invocation HTTP request, or via third-party storage or in-memory cache services, e.g., AWS S3, Google Cloud Storage, and AWS ElastiCache.

Inline transfers do not require external storage and can thus provide low latency, but pose limitations on the amount of data that can be transferred between function instances. Because invocation requests travel via the serverless autoscaling infrastructure, providers tend to restrict the maximum aggregate size of inlined payloads to reduce the pressure on the load balancer services,
% \boris{not clear if 'front-end' includes inter-function communication. What about 'load balancers' instead?}, 
which are shared across the datacenter.
% \boris{Discuss why the limitation exists. From  the intro: "Because invocation requests traverse the cloud provider's autoscaling infrastructure (i.e, the request {\em control plane}), providers limit the maximum size of inlined data to hundreds of KBs or a few MBs to mitigate the impact of large payloads on the forward logic along the request's path." Please integrate this message here. It's important, because it directly leads up to your LB scalability experiment.}
For instance, in AWS  Lambda, inline transfers are limited to 6MB and 256KB per HTTP request/response for synchronous and asynchronous invocation~\cite{aws:quotas}, respectively. 
% \dmitrii{TODO: argue that inline does not scale and does not support the reduce pattern}

In contrast to inline transfers, {\em through-storage} transfers can be used for arbitrarily large objects but require the use of an external storage service. 
For example, in AWS, a function {\em A} that needs to pass a large object as an input to function {\em B} would first save the object in an S3 bucket and pass the corresponding S3 key to {\em B}, which would then retrieve the object. 
% \boris{Add a sentence summarizing how that works.} 
Problematically, the use of a storage service adds latency in the critical path of communication and incurs an additional monetary cost to the developer. 
% For example, AWS S3, often used for cold storage, is billed at around \$0.02 per GB-month~\cite{s3:pricing} while a faster, in-memory AWS ElastiCache costs \$0.02 per GB-{\em hour}~\cite{elasticache:pricing}. Although seemingly small, in practice, storage expenses can easily dominate the overall cost of executing serverless applications, as we show in \S\ref{sec:workload_perf}.

The highest-performance alternative to a storage service in today's clouds that is not limited in the amount of data that can be transferred is an in-memory caching service, such as AWS ElastiCache. While offering lower latency and higher bandwidth than storage, ElastiCache comes with a significant cost overhead. For example, as of this writing, AWS S3 storage service is billed at around \$0.02 per GB-month~\cite{s3:pricing}, whereas ElastiCache costs \$0.02 per GB-{\em hour}~\cite{elasticache:pricing} -- a cost difference of around 700\tms{}. Moreover, these costs can easily dominate the overall cost of executing serverless applications. Indeed, as we show in \S\ref{sec:workload_perf}, data transferring can cost nearly 1000\tms{} more than compute time in AWS Lambda when using ElastiCache and 3\tms{} more if using AWS S3. In addition to their cost premium, another disadvantage of in-memory caches compared to storage is their lack of durability; users can set up replication for high availability, but that will further drive up the cost. Finally, neither self-hosted (e.g., on an AWS EC2 node) nor managed caching services support autoscaling by default, meaning that application developers must add that functionality themselves.


% \edb{DEDICATE A FULL PARAGRAPH TO ElastiCache.... this is a pretty fundamentally different solution from S3} 
% \boris{I agree with Ed. Here's what I would do: drop all references to EC in the paragraph right above (which will also avoid confusion as to why you're not considering EC in Fig 2), and dedicate a new paragraph, here, to EC. You need to discuss cost/perf as well as the complexity of EC in terms of engaging another (3rd) service. For the latter, you could point out that EC can be managed by AWS, but that adds further cost, or by the user, which necessarily adds complexity and provides another point of failure. }


\begin{figure}[t]
\subfloat[Average latency (lower is better).] {
       % \hspace{6pt}
        \includegraphics[width=0.49\columnwidth]{figures/background/latency-EC.png}
        \label{fig:back_latency}}
% \newline
\centering
\subfloat[Effective BW (higher is better).] {
        \includegraphics[width=0.49\columnwidth]{figures/background/bandwidth-EC.png}
        \label{fig:back_bw}}
% \newline
\centering
\caption{Latency and effective bandwidth characteristics of a single data transfer, inline and via AWS S3, and AWS ElastiCache (EC), in AWS Lambda. All axes are logarithmic.
}
\label{fig:back_char}
\end{figure}

% Fig.~\ref{fig:back_char} shows latency and effective bandwidth achieved with (synchronous) inline and through-storage data transfers in AWS Lambda. We obtained these results by instrumenting a pair of AWS Lambda functions, one invoking the other and passing payloads of various sizes with timestamps in user code. These timestamps capture both invocation and data transfer latencies, including those for S3 in through-storage transfers. We observe that the inline data transfers show lower latency and deliver higher bandwidth than the storage-based alternative. For instance, for a 100KB transfer, inline achieves 4.3\tms{} lower latency than through-storage. Crucially, Lambda users are limited to 6MB for inline transfers at most. Larger objects require the use of through-storage transfers.

Fig.~\ref{fig:back_char} shows latency and effective bandwidth achieved with synchronous inline transfers and those via AWS S3 and ElastiCache for Redis in AWS Lambda. We obtained these results by instrumenting a pair of AWS Lambda functions, one invoking the other and passing payloads of various sizes with timestamps in user code. These timestamps capture both invocation and data transfer latencies, including those for S3 and ElastiCache in the respective experiments. We observe that the inline data transfers deliver lower latency and higher bandwidth than the storage-based alternative. 
For instance, for a 100KB transfer, inline achieves 8.1\tms{} and 1.3\tms{} lower latency than S3 and ElastiCache, respectively. However, Lambda users are limited to 6MB maximum object size for inline transfers. Larger objects require the use of through-storage transfers.


\subsubsection{Research Proposals}
\label{sec:prior-research}

To overcome the limitations of inter-function communication methods used in production clouds, recent works have considered two alternative strategies. 
%namely using a smart and autoscaling third-party services and workarounds that enable direct IP transfers. 
The first strategy focuses on improving the performance of data transfers through the use of tiered storage.
For example, Locus~\cite{pu:shuffling} uses different storage tiers for specific purposes, namely Redis for shuffling and S3 for cold storage.
Pocket~\cite{klimovic:pocket} and SONIC~\cite{mahgoub:sonic} employ a similar idea and develop a control-plane solution to multiplex different storage services based on inferred application needs.
% \boris{I can't parse the following sentence.} 
Faa\$T\cite{romero:faast}, Cloudburst~\cite{sreekanti:cloudburst}, 
% FaasCache~\cite{DBLP:conf/asplos/FuerstS21}, 
and OFC~\cite{mvondo:ofc} propose using key-value stores
%, which scale their resources automatically according to the latency and throughput needs of serverless functions, 
as a cache for ephemeral data transfers.

While an improvement on production offerings, approaches that rely on one or more storage layers for data transfers fundamentally increase system complexity, impose additional coordination overheads at the application level, and incur latency cost in the critical path for writing and reading data. 
%by allowing both compute and storage autoscaling to co-exist without coordination.
% \boris{Rewrote the prev sentence. I don't think we need the next one - suggest drop.}
% In case the storage requirements need to be accounted for, the scheduling and placement decisions will become more challenging since the autoscaler has to add storage bandwidth and space into the placement decision process.


The second strategy advocated in research papers is to implement direct communication between function instances by exposing IP endpoints to functions~\cite{thomas:particle,wawrzoniak:boxer,nesterov:floki}.
% \boris{I'm not convinced the following is useful. XDT also requires infrastructure support. I'd instead jump straight to the next para from here.}
% While effective, such approaches pose significant impediments to adoption. Existing serverless infrastructure has not been designed with such functionality in mind, making this class of solutions harder to adopt.
% Particle~\cite{thomas:particle}, for example, evaluates the performance and implications of direct IP communication for serverless platforms and suggests extensions to the network layer to accommodate such transfers. 
% Boxer~\cite{wawrzoniak:boxer} suggests to use a NAT hole punching technique to enable direct IP communication. 
% \boris{rewrote the following para.}
Problematically, the unmediated direct IP communication between serverless instances introduces several issues. 
First, exposing IP addresses of the instances to untrusted user code is a security concern. Indeed, allowing a malicious user to infer serverless cloud network topology can facilitate denial-of-service and side channel attacks.
Secondly, communication using static IP addresses impedes the autoscaler from scaling individual functions independently and places the burden of load-balancing on the user. 
% Secondly, direct IP communication in the way it is currently implemented \boris{by 'currently implemented' do you mean in existing research proposals? Please clarify.} prevents the autoscaler to scale individual functions independently and places the burden of load balancing on the user. 
Indeed, doing so is fundamentally at odds with the autoscaling principle of serverless computing, and is thus highly unattractive for practical usage. 
%First, the user becomes responsible for balancing the load associated with data communication, e.g., if functions distribute jobs.
%Specifically, direct IP communication in the way it is currently implemented prevents the autoscaler to scale different functions independently.



% How this breaks autoscaling: a function can have any number of instances from 0 to virtually infinity. Consider an example (TODO: fig?) of a producer and a consumer functions, the former calling the latter; any of the producer instances should be able to call any consumer instances. This rules out sticky routing, e.g., opening a TCP socket, as an option because it would make autoscaling impossible.

% Both directions above, despite improving upon the production offerings, they have their own limitations.
% The external autoscaling storage approaches increase the overall system complexity by allowing both compute and storage autoscaling to co-exist without coordination.
% In case the storage requirements need to be accounted for, the scheduling and placement decisions will become more challenging since the autoscaler has to add storage BW and space into the placement decision process.


% The unmediated direct IP communication in serverless, on the other hand, has several issues.  First, the user becomes responsible for balancing the load associated with data communication, e.g., if functions exchange jobs.
% Specifically, direct IP communication in the way it is currently implemented prevents the autoscaler to scale different functions independently.
% Second, exposing IP addresses of the instances to untrusted user code is a security concern.
% For instance, allowing a malicious user to infer serverless cloud network topology can be of help in denial-of-service or side channel attacks.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
The goals are (might be in a different order): 
\begin{itemize}
    \item Support both pass-by-value and pass-by-reference API.
    \item High perf
    \item Keep provider information, like the IP addresses of function instances, transparent to the user code.
    \item Should be co-designed with the autoscaling infra, making communication bandwidth a load metric in addition to the inbound queue depth (in Knative; currently we don't talk much about this metric, maybe we should).
\end{itemize}



Despite the growing serverless computing popularity, serverless application scope is currently limited to stateless and compute-intensive applications, particularly, due to inefficient data communication in modern serverless clouds~\cite{hellerstein:serverless,jonas:cloud}. We argue that the cortex of the problem lies in the requirement of designing data communication support in conjunction with the serverless autoscaling infrastructure, limiting the performance of the existing approaches in production clouds or leading to a significant increase of the overall system complexity.

% \dmitrii{unstructured as of now but important thoughts}
% Fundamental issues with provider-based autoscaling. First, autoscaling restricts the developers to using {\em stateless} functions. 
% This requirement however results in the lack of efficient support for data communication, particularly the stateless nature of the functions don't allow them to freely exchange or share data. 
% Stateless nature of the functions prevents existing systems from supporting effective data communication and sharing.


\dmitrii{a paragraph on required API for the patterns like invoke and reduce. Most transferred data is ephemeral, as in inputs and outputs that are produced and consumed once, ~\cite{klimovic:understanding}. functions either invoke one another, sending invocation arguments, or reducing the outputs coming from many producers~\cite{fouladi:laptop,jonas:cloud}.
}


Existing systems support inline and storage-based transfers. Inline are low latency but low BW. Storage is higher BW but high latency. 
\dmitrii{how deep should we go in the baseline evaluation here?}

\marios{use qualitative args for inline, namely the 4MB/10MB constraint in AWS/Google and the LB load bottleneck; then show the latency and BW for S3 (have a figure, check the IISWC draft)}


% The cortex of the problem is that functions are abstract with ephemeral function instances hidden by the LB. Hence, the LB and the autoscaler are the crucial components (i.e., cannot be bypassed).


\\

Takeaway: data communication should be co-designed with the autoscaling infra, particularly with the LB.

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{State-of-the-Art Data Communication Mechanisms}




\subsubsection{Inline Transfers}


% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}[b]{0.49\linewidth}
%         \includegraphics[width=\linewidth]{figures/transfer/AWS Inline Transfer Latency.pdf}
%         \caption[size=18]{Median (solid) and tail (dashed) latencies}
%         \label{fig:inline-sizes}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.49\linewidth}
%         \includegraphics[width=\linewidth]{figures/transfer/inline.pdf}
%         \caption{Latencies for 10KB (solid) and 1MB (dashed) payload transfers}
%         \label{fig:inline-cdf}
%     \end{subfigure}
%     \caption[]{Inline data transfer latency as a function of payload size. Note that both axes in (a) and the X-axis in (b) are logarithmic.}
%     \label{fig:inline}
% \end{figure}


Inline transfers go thru the LB. Relatively low latency but very low BW  $<$264Mb/s (AWS). 


\subsubsection{Storage-based Transfers}

Storage transfers: higher, scalable BW but high tail latency. 

% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}[b]{0.49\linewidth}
%         \includegraphics[width=\linewidth]{figures/transfer/AWS Storage Transfer Latency.pdf}
%         \caption[size=18]{Median (solid) and tail (dashed) latencies}
%         \label{fig:storage-sizes}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.49\linewidth}
%         \includegraphics[width=\linewidth]{figures/transfer/storage.pdf}
%         \caption{Latencies for 1MB (solid) and 1GB (dashed) payload transfers}
%         \label{fig:storage-cdf}
%     \end{subfigure}
%     \caption[]{Storage-based data transfer latency as a function of payload size. Note that both axes in (a) and the X-axis in (b) are logarithmic.}
%     \label{fig:storage}
% \end{figure}

\subsubsection{Ephemeral storage}

Designing scalable storage is hard and/or expensive. Systems like CloudBurst and Pocket complicate the overall design. 

\subsubsection{Communication Fabrics Design Goals}

\begin{itemize}
    \item co-designed with the serverless autoscaling infra.
    \item no third-party components for the payloads
\end{itemize}

%%%%%%%%%%%%%%%%%%% EXAMPLE FIG
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/queuing/servicetime-across-providers-CDF-100000.pdf}
    \caption{Latency CDFs for different request burst sizes, arriving with a long IAT, for the functions with 1-second long execution time.}
    \label{fig:queuing}
\end{figure}


\end{comment}


==> old6-eval-osdi.tex <==
\section{Evaluation}
\label{sec:eval}

We evaluate \shortn{} in three steps. First, we conduct two sensitivity studies to find a best-performing configuration. Second, we study \shortn{} scalability in various communication scenarios using microbenchmarks while measuring latency and bandwidth. Finally, we evaluate \shortn{} against the baseline on three real-world serverless applications.

\subsection{\shortn{} Sensitivity Studies}
\label{sec:sensitivity}

\boris{I question the need for this section. If we're dropping CT, there's no need for 7.1.1. And 7.1.2 basically shows such low sensitivity, that it's not interesting -- the key points can be summarized in one paragraph in the Methodology.}

The implementation of \shortn{} leaves a few design choices for empirical evaluation, namely the choice of the streaming mechanism -- store-and-forward~(SF) vs. cut-through~(CT) -- as well as the depth of the \shortn{} buffers in the queue proxies. Both choices are important for supporting the \texttt{invoke()} API efficiently. We study the latency and effective bandwidth of \texttt{invoke()} in the single producer-consumer scenario~({\em 1-1)} while varying the streaming mechanism and QP buffer depth.


\subsubsection{The Streaming Mechanism} 

% is the first design choice that we investigate. 
We start by investigating the efficiency of the \stfw{} and CT streaming mechanisms.
Fig.~\ref{fig:eval_1-1} shows the latency and effective bandwidth of \shortn{} configurations using \stfw{} and CT streaming, varying the size of the transferred objects from 10KB to 100MB. Next, we compare these results to the configurations that use AWS S3 and inline transfers.\footnote{Note that the latencies of inline and S3-based transfers are slightly different from the ones presented in Fig.~\ref{fig:back_char}, as we deploy our serverless clusters on an EC2 node, not in AWS Lambda, and use the Knative load balancer instead of AWS.}

\begin{figure}[t!]
\subfloat[Latency (lower is better)] {
       % \hspace{6pt}
        \includegraphics[width=0.49\columnwidth]{figures/eval-ubench/lat_1-1.png}
        \label{fig:eval_1-1_lat}}
%\newline
\centering
\subfloat[Bandwidth (higher is better)] {
        \includegraphics[width=0.49\columnwidth]{figures/eval-ubench/bw_1-1.png}
        \label{fig:eval_1-1-lat}}
\newline
\centering
\caption{Average latency and effective bandwidth of the {\em 1-1} workflow, sweeping the transferred object size.
% \dmitrii{\shortn{} CT to be re-run with 1MB buffers}
% \dmitrii{ADD INLINE HERE}
}
% \vspace{-15pt}
\label{fig:eval_1-1}
\end{figure}

We observe that both \shortn{} configurations exhibit significantly lower latency and higher bandwidth than the configuration that uses S3. The gap between \shortn{} and S3 grows when increasing the object size. The \stfw{} configuration delivers 3.2$\times$ and 5.6$\times$ lower latency when transferring 10KB and 100MB objects, respectively, yielding up to 306MB/s effective bandwidth vs. 117MB/s peak S3 configuration bandwidth. This demonstrates better bandwidth scaling of \shortn{} with the size of the object, compared to S3.

Compared to \stfw, the cut-through streaming optimization accelerates \shortn{} by 1.1\tms{} for 10KB objects and 2.8\tms{} for 100MB objects, yielding 3.6-15.7\tms{} lower latency than with AWS S3. With a 100MB object, the \shortn-CT is able to deliver 855MB/s bandwidth, which is within 13\% of the bandwidth of vanilla gRPC streaming between two endpoints, communicating over a localhost interface. This result highlights the efficiency of the \shortn-CT design, which we use in all further experiments referring to it simply as \shortn{}.

Compared to \shortn{}, inline transfers are 1.9-3.8\tms{} faster and have higher  effective bandwidth.
%, \shortn{} delivers 1.9-3.8\tms{} higher latency and lower effective bandwidth. 
However, inline transfers impose a strict limitation on the maximum transfer size of $<$4MB in the gRPC/Knative setup and $<$6MB in AWS Lambda~\cite{aws:quotas}. In contrast, \shortn{} is not encumbered by object size limitations and supports large object transfers efficiently.
% with up to 2.8\tms{} higher bandwidth than the peak bandwidth of the inline transfers. \boris{than what??  Inline  has higher BW. I  think you should drop this phrase}.
Due to limitation on maximum object size for inline transfers, the rest of the evaluation does not consider this option. However, we note that for workloads that only transfer small objects and are limited to the 1-1 and scatter communication patterns, inline transfers represent a superior choice.

%second, showing the traces (aggregated, not Zipkin) for 10MB transfer.

\subsubsection{Memory Requirements for \shortn{}}
% Queue-Proxy's \shortn{} Buffer Depth
\label{sec:eval-memory}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.85\columnwidth]{figures/eval-ubench/lat_buffer_depth.pdf}
    \caption{Average latency of \shortn{} \texttt{invoke(}) for objects of various size, as a function of queue proxy~(QP) buffer depth.
    }
    % \vspace{-15pt}
    \label{fig:lat_buffer}
\end{figure}

Next, we evaluate the added memory overhead for blocking \shortn{} transfers, as non-blocking transfers do not require extra bookkeeping~(\S\ref{sec:xdt-api}).
% \boris{I did not see a discussion of buffering for async transfers in the design/implementation sections.} MOVED TO 4.2.1 (prog model)
% is the second design choice that is a subject to an empirical study.
Fig.~\ref{fig:lat_buffer} shows the average transfer latency for three object sizes, namely 1MB, 10MB, and 100MB. We vary the buffer depth from 64KB, which holds a single object chunk, to 4MB, which holds 64 chunks per buffer. 

Increasing the buffer size leads to a small decrease in the latency, leading us to conclude that the sensitivity of the \shortn{} design to buffer depth is small. For instance, transferring 1MB object with the buffer sizes of 64KB and 4MB is performed in 15ms and 16ms, respectively. The latency gap for transferring a 100MB object is slightly larger, with 270ms for a 64KB buffer size and 243ms for a 4MB buffer.

Based on the obtained results, we configure \shortn{} to use 1MB buffers in further experiments, as this size yields low latency for larger transfers, e.g., 250ms for a 100MB object, while imposing a relatively small memory overhead.
%(for example, the footprint of the AWS Firecracker hypervisor is \textasciitilde5MB~\cite{agache:firecracker}).

% \dmitrii{TODO} for xdt.Invoke. Sensitivity is low, slightly higher for 10MB objects. Hence, buffers can be shallow. In further experiments, we will use 1MB buffers. 



\subsection{Microbenchmarks}
\label{sec:ubenches}

This subsection further quantifies the latency and effective bandwidth characteristics of \shortn{} in common communication scenarios~(\S\ref{sec:method_ubenches}): 1-1, gather, scatter, and broadcast.

\subsubsection{Transfer Latency}

\begin{figure}[t]
\subfloat[Latency CDFs for 1MB objects.] {
       % \hspace{6pt}
        \includegraphics[width=0.49\columnwidth]{figures/eval-ubench/tail_1-1.png}
        \label{fig:tail_cdfs}}
%\newline
\centering
\subfloat[Median and tail latency, sweeping the object size.] {
        \includegraphics[width=0.49\columnwidth]{figures/eval-ubench/tail_1-1_sweep.png}
        \label{fig:tail_sweep}}
\newline
\centering
\caption{Transfer latency cumulative distribution functions~(CDFs), median and tail (99\textsuperscript{-th} percentile) latencies for S3 and \shortn{} in the {\em 1-1} workflow.
}
% \vspace{-15pt}
\label{fig:eval_tail}
\end{figure}

Latency is a key metric for interactive, user-facing cloud services. We study the latency characteristics as a function of the transferred object size in the 1-1 producer-consumer scenario~(Fig.~\ref{fig:eval_tail}). 

Fig.~\ref{fig:tail_cdfs} shows the latency cumulative distribution functions~(CDFs) for \shortn{} and AWS S3 transferring 1MB objects. We observe that \shortn{} exhibits significantly lower median and tail (99\textsuperscript{-th} percentile) latency, i.e., by 8.9\tms{} and 6.5\tms{} respectively, when compared to the configuration that uses S3. This indicates that the \shortn{} architecture, and our implementation of it, is well-suited to latency-critical workloads, which are common in cloud.
%, due to its simple, modular architecture and implementation using gRPC streaming, a production high-performance network technology, running on top of TCP.

Fig.~\ref{fig:tail_sweep} shows the average and the tail latencies of the two configurations while varying the size of the transferred objects. We notice that \shortn{} consistently shows lower median and tail latencies, by 6.0-14.2\tms{} and 6.5-13.0\tms{} respectively, in comparison to S3.


\subsubsection{Gather Communication Pattern}
\label{sec:eval_reduction}

Gather, or reduce, is essential for applications with functions whose input is the output of several other functions and use the \texttt{put()}/\texttt{get()} API. We explore the latency and effective bandwidth of such transfers, sweeping the number of producers, i.e., the gather degree, from 1 to 32. 

\begin{figure}[t]
\subfloat[Latency (lower is better)] {
       % \hspace{6pt}
        \includegraphics[width=0.49\columnwidth]{figures/eval-ubench/lat_reduce.png}
        \label{fig:lat_reduce}}
% \newline
\centering
\subfloat[Bandwidth (higher is better)] {
        \includegraphics[width=0.49\columnwidth]{figures/eval-ubench/bw_reduce.png}
        \label{fig:bw_reduce}}
\newline
\centering
\caption{Average latency and effective bandwidth of the {\em gather} workflow.}
\label{fig:eval_reduce}
% \vspace{-15pt}
\end{figure}

Fig.~\ref{fig:lat_reduce} shows the average latency of \shortn{} and S3-based configurations while transferring small (10KB) and large (10MB) objects. For small objects, \shortn{} achieves 5.6-9.3\tms{} lower latency compared to S3. \shortn{} delivers effective bandwidth of up to 11.8MB/s vs. S3's peak of 2.1MB/s, as shown in Fig.~\ref{fig:bw_reduce}. For large object transfers, \shortn{} delivers 8.2-12.3\tms{} lower latency, compared to S3, and provides effective bandwidth of up to 2175MB/s vs 230MB/s for S3.
% \boris{fill in}. 


\subsubsection{Scatter Communication Pattern} 
\label{sec:eval_fanout}

Scatter, or map, is important when functions have a large fan-out of calls to other functions, passing the objects via the \texttt{invoke()} and the \texttt{put()}/\texttt{get()} APIs. We study the latency and effective bandwidth of these transfers~(fig.~\ref{fig:eval_fanout}), varying the number of consumers, i.e., the scatter degree, from 1 to 32. 

\begin{figure}[t]
\subfloat[Latency (lower is better)] {
       % \hspace{6pt}
        \includegraphics[width=0.49\columnwidth]{figures/eval-ubench/lat_fanout.png}
        \label{fig:lat_fanout}}
% \newline
\centering
\subfloat[Bandwidth (higher is better)] {
        \includegraphics[width=0.49\columnwidth]{figures/eval-ubench/bw_fanout.png}
        \label{fig:bw_fanout}}
% \newline
\centering
\caption{Average latency and effective bandwidth characteristics of the {\em scatter} workflow.
% \dmitrii{maybe, add inline}
}
% \vspace{-15pt}
\label{fig:eval_fanout}
\end{figure}

Fig.~\ref{fig:lat_fanout} demonstrates the latency characteristics of \shortn{} and S3-based systems in the scatter scenario. 
% \dmitrii{maybe, add inline} 
We observe that for small object transfers, \shortn{} consistently shows 1.8-3.7\tms{} lower latency over the S3-based baseline. \shortn{} delivers 0.5-3.6MB/s of effective bandwidth vs. 0.1-2.1MB/s for the S3-based system, as depicted in Fig.~\ref{fig:bw_reduce}. For large transfers, \shortn{} delivers 10.9-11.6\tms{} speedups for the low 1-4 scatter degree and more modest 2.4-4.9\tms{} speedups for the higher scatter degree of 8-16. For the scatter degree of 32, \shortn{} matches the performance of the S3-based configuration, indicating a performance bottleneck in our prototype that requires investigation. 
% provides 20\% higher latency than the S3-based configuration. We attribute this behavior to the fact that gRPC uses a single gRPC channel, i.e., a single HTTP/2 connection, between the producer function server and \rpprod{}, which saturates at around 700MB/s. We hypothesize that this inefficiency of our \shortn{} prototype can be eliminated by maintaining a pool of gRPC channels, i.e., HTTP/2 connections, as suggested in gRPC best practices~\cite{grpc:multiple-channels}. 


\subsubsection{Broadcast Communication Pattern} 
\label{sec:eval_brd}

Broadcast support is required for functions that distribute the same data among many consumers, via a single \texttt{put()} call followed by multiple \texttt{get()} calls with the {\em same} S3 key or \shortn{} reference. We investigate the performance characteristics of the \shortn{} and S3-based systems, sweeping the size of the transferred objects.

\begin{figure}[t]
\subfloat[Latency (lower is better)] {
       % \hspace{6pt}
        \includegraphics[width=0.49\columnwidth]{figures/eval-ubench/lat_broadcast.png}
        \label{fig:lat_brd}}
% \newline
\centering
\subfloat[Bandwidth (higher is better)] {
        \includegraphics[width=0.49\columnwidth]{figures/eval-ubench/bw_broadcast.png}
        \label{fig:bw_brd}}
% \newline
\centering
\caption{Average latency and effective bandwidth characteristics of the {\em broadcast} workflow.
}
\label{fig:eval_brd}
% \vspace{-15pt}
\end{figure}

Fig.~\ref{fig:eval_brd} demonstrates the latency and effective bandwidth characteristics of the \shortn{} and S3-based configurations. For both small and large objects, \shortn{} delivers 2.6-6.3\tms{} lower latency. The effective bandwidth of \shortn{} is particularly high when transferring large objects, reaching 3331MB/s vs. peak 590MB/s delivered by S3. 
%%%%%%%%% BUG%%%%%%%%
% The high bandwidth achieved by \shortn{} is due to the fact that the object's data are transferred from the producer function server to its \rpprod{} only once, which avoids the bottleneck that appears in the scatter scenario~(\S\ref{sec:eval_fanout}). Once \rpprod{} has the data buffered, it can immediately start broadcasting, using a separate gRPC channel for each consumer.  
% \boris{The scatter case doesn't discuss multiple data copies - it only talks about a single channel. For someone with my level of knowledge, that's not enough info to understand that data is copied many times.}

% Compared to the similar scatter experiment~(\S\ref{sec:eval_fanout}), both configurations scale much better, exhibiting almost linear effective bandwidth scaling~(Fig.~\ref{fig:bw_brd}). This observation supports our hypothesis that the \texttt{put()} call implementation is the bottleneck for \shortn{} in the scatter scenario. 
%%%%%%%%% BUG%%%%%%%%

% \subsection{\shortn{} Sensitivity Studies}

% Chunk size (we just say that 64K is recommended for up to large BW NICs; gRPC doesn't transfer extra bytes), buffer size, routing type.
% \textbf{InvokeWithXDT: buffer size sweep with 100KB and 10MB payloads}



% \textbf{Sweep payload size from 10KB to 100MB: Invoke and Get/Put}


\subsection{Real-World Workloads}

Next, we study three data-intensive applications (\S\ref{sec:method_apps}) and present their end-to-end latency along with a detailed breakdown of the sources of latency. 

\begin{figure}[t]
\subfloat[Video Analytics.] {
       % \hspace{6pt}
        \includegraphics[width=0.33\columnwidth]{figures/workloads/video_analytics.png}
        \label{fig:video}}
% \newline
\centering
\subfloat[Stacking Ens. Training.] {
        \includegraphics[width=0.33\columnwidth]{figures/workloads/stacking.png}
        \label{fig:stacking}}
% \newline
\centering
\subfloat[MapReduce.] {
        \includegraphics[width=0.33\columnwidth]{figures/workloads/mapreduce.png}
        \label{fig:stacking}}
% \newline
\centering
\caption{Latency breakdown of real-world workloads, deployed in \shortn{} and S3-based systems.
}
\label{fig:workloads}
\end{figure}

\textbf{Video Analytics} spends 30\% of its execution time in transferring the video fragment and the frames in the S3-based configuration. With \shortn{}, this fraction decreases to 19\%, yielding the overall speedup of 1.14\tms{} over the baseline. This speedup comes from 1.7\tms{} and 1.6\tms{} faster transmission of video and frames, respectively.

% \subsubsection{Stacking Ensemble Training} spends 61\% of execution time in data communication, when using S3 for data communication. The largest fractions of data communication are the {\em gather trained models} and the {\em meta-trainer put} phases, accounting for 39\% and 9\% of the overall execution time. Using \shortn{} allows to decrease both of these fractions to 17\% and 4\%, respectively, driving the overall data communication fraction to 31\%. Hence, \shortn{} delivers 1.89\tms{} speedup vs. the baseline that communicates via S3.

\textbf{Stacking Ensemble Training} spends 63\% of execution time in data communication in the S3-based baseline. The largest fractions of data communication are the {\em gather trained models} and the {\em meta-trainer put} phases, accounting for 39\% and 9\% of the overall execution time. Using \shortn{} allows to decrease both of these fractions to 12\% and 3\%, respectively, driving the overall data communication fraction down to 23\%. Thus, \shortn{} delivers a 2.71\tms{} speedup over the S3 baseline.
% \artemiy{I am not clear how 2.71\tms{} is calculated from the numbers above. Assuming that the execution time with S3 was X, the non-communication part with S3 is (1 - 0.63)X = 0.37X. I assume the execution time of the non-communication part does not change when switching to \shortn{}. With \shortn{} execution time is Y. From above, with \shortn{}, communication takes 23\%, then the rest (non-communication part) is 77\%. Thus, 0.77 * Y = 0.37 * X. Hence, Y = 0.48 X. Speedup is 2.08\tms{} but not 2.71\tms{} as specified above. Am I missing smth?}

\textbf{MapReduce} shows 63\% of execution time spent in communication for the S3 baseline. Moreover, 28\% of the overall time is spent retrieving the original input from S3 and writing back the results to S3, which we do not optimize with \shortn{}. The rest, i.e., 33\% of time, are subject to \shortn{} optimization. 
\shortn{} allows to achieve 1.42\tms{} overall speedup vs. the S3-baseline. Note, however, that we plot the latency breakdown of the critical path across a highly parallel job, i.e., the longest-running mapper and reducer invocations. \shortn{}'s speedup is achieved due to a significant decrease in data shuffling, namely mapper-put and the reducer-get phases, which are sped-up by 3.9\tms{} and 2.0\tms{} respectively.
% \footnote{We observe that the load imbalance across mappers and reducers leads to different critical paths for the S3 and \shortn-based configurations, particularly, leading to the slightly different mapper and reducer compute times as well as the mapper-get fraction, as compared to the S3-based configuration.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{itemize}
    \item video analytics
    \item mapreduce: scan and aggreg, maybe join
    \item stacking training
\end{itemize}


\textbf{TODO}:

\begin{itemize}
    \item Support elasticache. 
    \item Add load experiments for the microbenchmarks, maybe for the workloads as well.
\end{itemize}



\textbf{Optional but good to have}:

\begin{itemize}
    \item Tail latency: \shortn{} vs. S3.
    \item Use more than one worker node in Eval. %Maybe, use EKS.
    \item Implement the broadcast trees. 
\end{itemize}
\end{comment}


==> old7-discuss.tex <==
\section{Discussion}
\label{sec:discuss}

\dmitrii{
\shortn{} enables efficient transfer of ephemeral data across functions without adding cost or complexity to the application logic. By design, \shortn{} is much faster than transferring data via conventional storage services, such as AWS S3, because \shortn{} avoids unnecessary writing and reading to the durable tier of storage services, which incurs high latency overheads and carries a monetary cost. Compared to an in-memory cache, \shortn{} offers similar or better performance {\without} the staggering cost or complexity overheads associated with using an additional service. Our results show that the cost overheads of an in-memory cache are prohibitive, exceeding compute costs by one to two orders of magnitude (Table~\ref{tbl:cost}). Meanwhile, the use of an additional service for the caching tier burdens the developer with additional design complexity in the application logic and may require manual reconfiguration (or further application complexity) to accommodate changes in load or data volume. In contrast, \shortn{} avoids the need for an additional service and its bandwidth naturally scales with the number of producer and consumer instances. In line with the requirements articulated in Sec~\ref{??}, \shortn{} delivers high performance, compatibility with existing semantics and API, native autoscaling, and security. 


%Despite the lack of the durability guarantees, \shortn{} preserves the semantics of a serverless function invocation, exposing errors that may occur during an \shortn{} transfer to the application logic, e.g., to re-run a subset of functions in the application workflow. 

%\shortn{} offers on-par or better transfer speed when compared to a system equipped with an in-memory cache for transferring ephemeral data but without adding any cost or complexity of using an additional service for a data-intensive serverless application. \shortn{} can deliver a similar performance as an in-memory cache because it buffers payloads in the main memory of the producer function. However, this bookkeeping is free for both the application developer {\em and} provider because of the short ephemeral data lifetime and the extended lifetime of serverless function instances with their main memory reserved after them by the cluster infrastructure, as discussed in \S\ref{sec:design-insights}. Finally, cache services such as ElastiCache typically require manual re-configuration to accommodate changes in the demand for data transfer bandwidth, increasing the burden on application developers. In contrast, the bandwidth of \shortn{} transfers scales naturally with a number of producer and consumer instances.

%In conclusion, our work shows that data-intensive serverless applications can achieve high performance and low cost without deploying an intermediary service.
}

\begin{comment}
    
% \boris{This section reads like a Prior work section -- there is no real discussion, it's just compare and contrast of \shortn{} with prior work. I strongly feel it should be merged w next section.}

% \boris{This is too little. You need to focus on performance, and make a qualitative argument that \shortn{} can achieve same or better perf WITHOUT the need for a new tier of storage and its associated deployment complexity and cost.}
Prior work~\cite{klimovic:pocket,pu:shuffling,mahgoub:sonic,shillaker:faasm,sreekanti:cloudburst} considers a number of ephemeral storage service designs,
aiming to provide high-performance transfers without imposing a large cost. Hence, some works~\cite{klimovic:pocket,pu:shuffling,sreekanti:cloudburst,mvondo:ofc,romero:faast} feature a multi-tier design where the first tier comprises a fast, but pricey, in-memory store while the second tier is slow and cost-optimized. To reduce the cost of the pricey in-memory tier, some proposals~\cite{klimovic:pocket,mahgoub:sonic,mvondo:ofc} employ machine-learning techniques in the control plane for intelligent object allocation. Such approaches necessarily increasing the complexity of serverless infrastructure.
\dmitrii{Moreover, although intelligent tiered storage systems improve average delays of ephemeral data transfers, they inevitably expose the large latencies of the slower tiers in the tail latency, which undermines the quality-of-service of interactive applications commonly deployed in serverless clouds.}
% , fundamentally replicating the role of the autoscaling components that already exist for serverless compute (\S\ref{sec:autoscaling}). 

Another line of work employs direct inter-function communication approaches~\cite{wawrzoniak:boxer, thomas:particle} by exposing the IP addresses of function instances to the user code. Doing so increases the attack surface and places the burden of load balancing and scaling on the user. \boris{Need to make a bigger deal out of this -- reiterate the importance of autoscaling etc, the points that were made at the beginning of the paper.}
% \sout{aiming to provide seamless scalability and scaling that can match the autoscaling property inherent to the serverless compute infrastructure} \boris{this is a misplaced emphasis. You should focus on performance, which is the purpose of in-memory storage. Scalability can be an optional secondary point}. 



% In this work, we question the fundamental necessity of the ephemeral storage for data-intensive serverless design, 
% With \shortn{}, we qualitatively show that it is possible to achieve the performance of an in-memory data store, which is the peak performance configuration for ephemeral storage.} By design, the \shortn{} data-plane's performance is equivalent to a single direct data transfer initiated by the consumer side. 
% For compatibility with available storage service APIs, our \shortn{} prototype is implemented atop of gRPC (i.e., HTTP/2), which is a software-only fabric that imposes a relatively high CPU load. In contrast to using a storage service, \shortn{} can be seamlessly ported to a much more efficient hardware-accelerated fabric, e.g., using one-sided RDMA reads, minimizing CPU load imposed by the \shortn{} data plane to a handful of memory instructions. Note that \shortn{} is a part of the trusted provider infrastructure, giving the much desired flexibility and compatibility to the providers, which does not apply to the previously proposed direct communication approaches~\cite{wawrzoniak:boxer, thomas:particle}.

% \boris{I don't understand whether this paragraph is related to the first one (ephemeral storage) or RDMA one. You need paragraph headings.}

With \shortn{}, it is possible to obviate the need for ephemeral storage \textit{and} achieve the performance of an in-memory data store -- the peak storage performance configuration -- at the cost that is negligible compared to storage. By design, the performance of the \shortn{} data plane is equivalent to a single direct data transfer initiated by the consumer side. 
% \sout{\dmitrii{Furthermore, although our prototype is implemented atop the Cap'n Proto RPC fabric, the \shortn{} data plane can be optimized to the wire speed, e.g., by using RDMA, which would also reduce the CPU load imposed by communication.}} 
% \boris{I do not find the previous sentence useful, and bringing in CapnProto here is definitely not helpful.}
\boris{The following sentences are not related to each other. I could not follow them. I think you want to stress the fact that \shortn{} doesn't require an extra service (unlike EC) and has no added cost overhead, unlike S3 and EC.}
While prior work shows~\cite{klimovic:pocket,klimovic:understanding,pu:shuffling} that storage usage can be prohibitively expensive due to its pricey in-memory tier. 
\dmitrii{In contrast, \shortn{} requires no extra bookkeeping.}
% ATC'23 version: 
% In contrast, the cost of transmitting an object over \shortn{} is equivalent to the cost of 1MB bookkeeping per concurrent blocking transfer (\S\ref{sec:eval-memory}) \dmitrii{FIXME} for the duration of the transfer; and the data transferred via the non-blocking API requires no extra bookkeeping at all (\S\ref{sec:xdt-api}).
Finally, both performance and cost of \shortn{} scales naturally with the number of instances that perform \shortn{} transfers at any time. 
\end{comment}

% following the compute resources usage. Storage consists of long-running stateful services with considerable memory footprint that is the main reason for the high storage cost.  The added \shortn{} cost is proportional to the number of instances that perform \shortn{} transfers at any moment of time. 
% For such an instance, \shortn{} imposes a memory overhead of 1MB per concurrent blocking transfer, in a producer function instance's QP (\S\ref{sec:eval-memory}), whereas the data transferred via the non-blocking \texttt{get/put} API requires no extra bookkeeping (\S\ref{sec:xdt-api}).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
There have been many stores proposed for ephemeral data.

due to the direct mem-to-mem transfer, \shortn{} provides perf comparable with the fastest in-memory tier but doesn’t have their scalability, cost, and complexity limitations.



Although our prototype is sw-only atop of gRPC (HTTP/2), \shortn{} data plane can be optimized to the wire speed, e.g., by using RDMA, which would considerably reduce overall CPU cycles.

Summary: \shortn{} provides best perf, less CPU load, no added cost.
\end{comment}

\begin{comment}
\textbf{Economical and performance implications of \shortn{}.} Service developers are charged based on the memory utilization and the execution time during their functions' invocations. \shortn{} naturally fits this pricing model. For instance, the users may declare the number of concurrently transmitted objects per function using the synchronous interface and, particularly, the asynchronous interface, requiring deeper buffers. Then, a simple calculation can define the fixed-memory overhead, added by \shortn{}, that can be billed to the developers.


\textbf{HW support}. RDMA instead gRPC; put QP in SmartNIC; 


\textbf{\shortn{} applicability space}. Use inline where possible (?), use \shortn{} elsewhere

\textbf{Further producer bandwidth scaling.} broadcast trees







\textbf{CPU throttling}. Our eval doesn't cover it, however the vCPU count per func is growing.

\textbf{Integration with non-serverless services.} Possible to deploy a service with the \shortn{} SDK and an RP component, which may hold transmitted objects, for other functions to pull them from.

\end{comment}

